Normality Addition via Normality Detection in Industrial Image Anomaly Detection Models

The task of image anomaly detection (IAD) aims to identify deviations from normality in image data. These anomalies are patterns that deviate significantly from what the IAD model has learned from the data during training. However, in real-world scenarios, the criteria for what constitutes normality often change, necessitating the reclassification of previously anomalous instances as normal. To address this challenge, we propose a new scenario termed "normality addition," involving the post-training adjustment of decision boundaries to incorporate new normalities. To address this challenge, we propose a method called Normality Addition via Normality Detection (NAND), leveraging a vision-language model. NAND performs normality detection which detect patterns related to the intended normality within images based on textual descriptions. We then modify the results of a pre-trained IAD model to implement this normality addition. Using the benchmark dataset in IAD, MVTec AD, we establish an evaluation protocol for the normality addition task and empirically demonstrate the effectiveness of the NAND method.

==> texs/3_fig_normality_addition.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/na_problem.pdf}
    \vspace{-20pt}
    \caption{\textbf{A depiction of normality addition problem.} Leather의 color pattern을 정상으로 처리하기 위해, normality를 더한다. 기존의 anomaly detection model은 이를 anomaly로 잡지만, normality addition 결과 normal로 잘 나온다.}
    \vspace{-10pt}
    \label{fig:na_problem}
\end{figure}
